Optimization of Closed-Loop Shallow Geothermal Systems Using Analytical Models

Closed-loop shallow geothermal systems are one of the key technologies for decarbonizing the residential heating and cooling sector. The primary type of these systems involves vertical borehole heat exchangers (BHEs). During the planning phase, it is essential to find the optimal design for these systems, including the depth and spatial arrangement of the BHEs. In this work, we have developed a novel approach to find the optimal design of BHE fields, taking into account constraints such as temperature limits of the heat carrier fluid. These limits correspond to the regulatory practices applied during the planning phase. The approach uses a finite line source model to simulate temperature changes in the ground in combination with an analytical model of heat transport within the boreholes. Our approach is demonstrated using realistic scenarios and is expected to improve current practice in the planning and design of BHE systems.

==> nomenclature.tex <==
\begin{table*}[th!]
\footnotesize
\label{tab:nomenclature}
  \begin{framed}
  \nomenclature[M]{$\thermaldif$}{Thermal diffusivity [m$^2$/s]}
  \nomenclature[M]{$\thermalcond$}{Thermal Conductivity [W/(m K)]}
    \nomenclature[M]{$\beta$}{Normalized borehole conductance [-]}
       \nomenclature[M]{$\Psi$}{Local/Global Field Interaction term [K]}
        \nomenclature[M]{$\gamma$}{Borehole Characteristic parameter [-]}
  \nomenclature[L, B]{$\nbhe$}{Number of Boreholes [-]}
  \nomenclature[L, B]{R}{Resistance}
  \nomenclature[L, m]{$\flowrate$}{Flow rate [kg/s]}
    \nomenclature[L, T]{$T$}{Temperature [K]}
  \nomenclature[L, c]{$c$}{Specific heat capacity [J/(kg $\cdot$ K)]}
  \nomenclature[L, L]{$\length$}{Length of the Boreholes [m]}
  \nomenclature[L, x]{$x,y$}{Horizontal coordinates [-]}
  \nomenclature[L, z]{$z$}{Vertical coordinate [-]}
  \nomenclature[L, p]{$\positions$}{Positions of BHE [-]}
  \nomenclature[S]{$k,\hat k$}{Counter for BHEs}
  \nomenclature[S]{$r$}{Refrigerant}
  \nomenclature[L, q]{$\heatextr$}{Heat extraction rate per unit length [W/m]}
  \nomenclature[F]{$\green$}{Green's Function}
  \nomenclature[F]{$\verticalkernel$}{Vertical Kernel}
  \nomenclature[F]{$\horizontalkernel$}{Horizontal Kernel}
    \nomenclature[F]{$\mathcal{T}$}{Simulation end time [s]}
  \nomenclature[L, rb]{$\bheradius$}{Borehole radius}
  \nomenclature[M]{$\density$}{Density [kg/m$^3$]}
  \nomenclature[S]{inter}{pipe-to-pipe connection}
    \nomenclature[S]{s}{soil-to-pipe connection}
\nomenclature[S]{$^\circ$}{interior of a set}
  
    % \nomenclature[L, B]{$B$}{Saturated aquifer thickness [m]}
    % \nomenclature[L, n]{$n_{\mathrm{doublet}}$}{Number of installed doublets in city block [-]} 
    % \nomenclature[M]{$\alpha$}{Hydraulic breakthrough parameter [m$^2$/s]} 
    % \nomenclature[M]{$\chi$}{Line length [m]}
    % \nomenclature[M]{$\Delta$}{Distance between two wells or two doublets [m]}
    % \nomenclature[M]{$\Delta_\mathrm{min}$}{Regulatory minimum distance [m]}
    % \nomenclature[L, m]{$m$}{Interference parameter [m]}    
    % \nomenclature[L, x]{$x, y$}{Coordinates of a well [m]}
    % \nomenclature[S]{$j$}{Counter for extraction wells}
    % \nomenclature[S]{$i$}{Counter for injection wells}
    % \nomenclature[S]{$k, p$}{Counters for doublets}
    % \nomenclature[S]{$\mathrm{ext}$}{Extraction}
    % \nomenclature[S]{$\mathrm{inj}$}{Injection}
    % \nomenclature[S]{$\mathrm{min}$}{Minimum}
    % \nomenclature[S]{$\mathrm{max}$}{Maximum}
    % \nomenclature[S]{$\tilde{a}$}{Median of $a$}
    % \nomenclature[L, u]{$\boldsymbol{u}$}{Optimization variables}
    % \nomenclature[L, g1]{$\mathbf{g}_1$}{Equality constraints}
    % \nomenclature[L, g2]{$\mathbf{g}_2$}{Inequality constraints}    
    %\nomenclature{\mbox{}}{}
    \printnomenclature
  \end{framed}
\end{table*}
